Edge Computing in Distributed Acoustic Sensing: An Application in Traffic Monitoring

Distributed acoustic sensing (DAS) technology leverages fiber optic cables to detect vibrations and acoustic events, which is a promising solution for real-time traffic monitoring. In this paper, we introduce a novel methodology for detecting and tracking vehicles using DAS data, focusing on real-time processing through edge computing. Our approach applies the Hough transform to detect straight-line segments in the spatiotemporal DAS data, corresponding to vehicles crossing the Astfjord bridge in Norway. These segments are further clustered using the Density-based spatial clustering of applications with noise (DBSCAN) algorithm to consolidate multiple detections of the same vehicle, reducing noise and improving accuracy. The proposed workflow effectively counts vehicles and estimates their speed with only tens of seconds latency, enabling real-time traffic monitoring on the edge. To validate the system, we compare DAS data with simultaneous video footage, achieving high accuracy in vehicle detection, including the distinction between cars and trucks based on signal strength and frequency content. Results show that the system is capable of processing large volumes of data efficiently. We also analyze vehicle speeds and traffic patterns, identifying temporal trends and variations in traffic flow. Real-time deployment on edge devices allows immediate analysis and visualization via cloud-based platforms. In addition to traffic monitoring, the method successfully detected structural responses in the bridge, highlighting its potential use in structural health monitoring.

==> sections/bin.tex <==
Yes, there is a general approach to calculate the area between two lines (or more generally, two functions) over a given interval \([a, b]\), regardless of whether the lines intersect within that interval. The key is to account for the possibility of the lines crossing each other, which changes which function is on top.

The general formula for the area \(A\) between two functions \(f(x)\) and \(g(x)\) over the interval \([a, b]\) is:

\[
A = \int_{a}^{b} |f(x) - g(x)| \, dx
\]

This formula uses the absolute value \( |f(x) - g(x)| \) to ensure that the area is always positive, regardless of which function is on top. Here's how you can apply it:

1. **Define the Functions:**
   - \(f(x)\) and \(g(x)\) represent the equations of the two lines.
   - Example: \(f(x) = m_1x + b_1\) and \(g(x) = m_2x + b_2\).

2. **Determine the Interval:**
   - The interval \([a, b]\) can be any range where you want to calculate the area.

3. **Integrate Using Absolute Value:**
   - Compute the integral of the absolute difference between the two functions over the interval \([a, b]\).

### Example with General Formula

Let's consider two lines:
- \(f(x) = 2x + 1\)
- \(g(x) = -x + 4\)

We want to find the area between these lines from \(x = 0\) to \(x = 3\).

1. **Set Up the Integral:**
   \[
   A = \int_{0}^{3} |(2x + 1) - (-x + 4)| \, dx
   \]
   \[
   A = \int_{0}^{3} |3x - 3| \, dx
   \]

2. **Handling Absolute Value:**
   Determine the points where \(f(x) = g(x)\) to split the integral where necessary (if the lines intersect within the interval):
   \[
   3x - 3 = 0 \implies x = 1
   \]

   So, we split the integral at \(x = 1\):
   \[
   A = \int_{0}^{1} (3x - 3) \, dx + \int_{1}^{3} -(3x - 3) \, dx
   \]

   The negative sign in the second integral accounts for the absolute value when \(3x - 3 < 0\) (i.e., when \(g(x) > f(x)\)).

3. **Compute the Integrals:**

   For \(0 \le x \le 1\):
   \[
   A_1 = \int_{0}^{1} (3x - 3) \, dx = \left[ \frac{3x^2}{2} - 3x \right]_{0}^{1}
   \]
   \[
   A_1 = \left( \frac{3}{2} - 3 \right) - 0 = -\frac{3}{2}
   \]

   For \(1 \le x \le 3\):
   \[
   A_2 = \int_{1}^{3} -(3x - 3) \, dx = -\left[ \frac{3x^2}{2} - 3x \right]_{1}^{3}
   \]
   \[
   A_2 = -\left( \frac{27}{2} - 9 - \left(\frac{3}{2} - 3\right)\right)
   \]
   \[
   A_2 = -\left( \frac{27}{2} - 9 - \frac{3}{2} + 3\right)
   \]
   \[
   A_2 = -\left( \frac{27}{2} - \frac{3}{2} - 6 \right)
   \]
   \[
   A_2 = -\left( 12 - 1.5 \right)
   \]
   \[
   A_2 = -10.5
   \]

4. **Calculate Total Area:**

   Since area cannot be negative, we take the absolute values of the areas:
   \[
   A = |A_1| + |A_2|
   \]
   \[
   A = \frac{3}{2} + 10.5 = 12 \text{ square units}
   \]

This general approach ensures that you always get the correct area between the two curves (lines) over the given interval, accounting for any crossings or intersections between the functions.
